CasimirRFM: A Mathematica package for Riemann-flat compactifications with Casimir energies

CasimirRFM is a Mathematica package for the study of compactifications on Riemann-flat manifolds and the computation of one-loop Casimir energies in higher-dimensional field theories and supergravity. It implements an efficient numerical evaluation of lattice sums using Ewald summation, and computes both lower-dimensional Casimir potentials and local higher-dimensional Casimir energy densities, allowing for general massless spectra and twisted boundary conditions. The package provides tools for constructing and analysing the finite groups defining these manifolds, determining invariant metrics and cohomology bases, identifying compatible spin structures, and computing moduli-space metrics. Moreover, it evaluates the traces of holonomy elements in the graviton, $p$-form, spinor, and Rarita-Schwinger representations. We describe the mathematical formulation and numerical implementation of the package, and illustrate its use through a compactification of Type IIB supergravity on $T^6/\mathbb{Z}_8$, including the computation of the Casimir potential and the visualization of localised Casimir-brane contributions.

==> package-summary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Package Summary 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagebreak 
\begin{mdframed}[
    linewidth=1pt,
    roundcorner=2pt,
    innertopmargin=2em, 
    innerbottommargin=1em, 
    innerleftmargin=2em,
    innerrightmargin=2em] 
    
    \begin{center} 
        {\Large\bfseries Package Information} 
    \end{center} 
    
    \vspace{2em} 
    \hspace{-1em}
    \begin{tabular}{p{0.2\textwidth} p{0.8\textwidth}} 
        \textbf{Name} & \texttt{CasimirRFM} \\[0.2cm] 
        \textbf{Version} & 1.0 \\[0.2cm] 
        \textbf{Release Date} & July 2026 \\[0.2cm]
        \textbf{Repository} & \url{https://github.com/bruno-valeixo-bento/CasimirRFM} \\[0.2cm] 
        \textbf{License} & MIT License \\[0.2cm] 
        \textbf{Requirements} & Mathematica 13.0 or later \\[0.2cm] 
        \textbf{Author} & Bruno Valeixo Bento \\[0.2cm] 
    \end{tabular} 
    \vspace{0.4cm} 
    
    \noindent
    \textbf{Description:} 
    \texttt{CasimirRFM} is a Mathematica package for the study of compactifications on Riemann-flat manifolds (RFMs) and the computation of one-loop Casimir energies in higher-dimensional field theories and supergravity models. 
    \begin{itemize} 
        \item Construction and analysis of finite groups defining RFMs; computation of invariant metrics, cohomology forms, and spin structures. 
        \item Efficient numerical evaluation of lattice sums using Ewald summation; computation of Casimir potentials and Casimir energy densities. 
        \item Evaluation of Lorentz-group traces in graviton, $p$-form, spinor and Rarita--Schwinger representations. 
    \end{itemize} 
    \vspace{0.2cm} 

    \noindent
    \textbf{Citation:} 
    If you use \texttt{CasimirRFM} in scientific work, please cite 
    \begin{quote} 
        B.~Valeixo Bento, \emph{CasimirRFM: A Mathematica package for Riemann-flat compactifications with Casimir energies}, Version 1.0 (2026), \url{https://github.com/bruno-valeixo-bento/CasimirRFM}
    \end{quote} 
    and the accompanying methodology paper \cite{ValeixoBento:2025yhz}
    \begin{quote} 
        B.~Valeixo Bento and M.~Montero, \emph{An M-theory dS maximum from Casimir energies on Riemann-flat manifolds}, JHEP \textbf{01} (2026) 099, arXiv:2507.02037
    \end{quote} 
    \vspace{0.2cm} 
\end{mdframed}
